Macroscopic DNA-programmed photonic crystals via seeded growth

Photonic crystals -- a class of materials whose optical properties derive from their structure in addition to their composition -- can be created by self-assembling particles whose sizes are comparable to the wavelengths of visible light. Proof-of-principle studies have shown that DNA can be used to guide the self-assembly of micrometer-sized colloidal particles into fully programmable crystal structures with photonic properties in the visible spectrum. However, the extremely temperature-sensitive kinetics of micrometer-sized DNA-functionalized particles has frustrated attempts to grow large, monodisperse crystals that are required for photonic metamaterial applications. Here we describe a robust two-step protocol for self-assembling single-domain crystals that contain millions of optical-scale DNA-functionalized particles: Monodisperse crystals are initially assembled in monodisperse droplets made by microfluidics, after which they are grown to macroscopic dimensions via seeded diffusion-limited growth. We demonstrate the generality of our approach by assembling different macroscopic single-domain photonic crystals with metamaterial properties, like structural coloration, that depend on the underlying crystal structure. By circumventing the fundamental kinetic traps intrinsic to crystallization of optical-scale DNA-coated colloids, we eliminate a key barrier to engineering photonic devices from DNA-programmed materials.

==> tableFacetAngles.tex <==
d (nm) & $\alpha_{110}$ & $\beta_{110}$ & $\alpha_{101}$ & $\beta_{101}$ \\
\hline

250 & 109.5\pm0.4 & 125.3\pm0.4 & 109.5\pm0.4 & 125.3\pm0.4\\
430 & 106.2\pm1.6 & 126.9\pm0.8 & 111.1\pm0.8 & 124.4\pm0.4 \\
600 &  97.0\pm1.9 & 131.5\pm1.0 & 116.0\pm1.1 & 122.0\pm0.5 

==> unusedBibSources.tex <==

@Article{Nozawa2018,
  author        = {Nozawa, Jun and Uda, Satoshi and Guo, Suxia and Toyotama, Akiko and Yamanaka, Junpei and Okada, Junpei and Koizumi, Haruhiko},
  title         = {Step Kinetics Dependent on the Kink Generation Mechanism in Colloidal Crystal Growth},
  journal       = {Crystal Growth \& Design},
  year          = {2018},
  volume        = {18},
  number        = {5},
  pages         = {2948--2955},
  month         = may,
  issn          = {1528-7483},
  comment       = {doi: 10.1021/acs.cgd.8b00063},
  doi           = {10.1021/acs.cgd.8b00063},
  publisher     = {American Chemical Society},
}

@article{zhang2016self,
  title={Self-assembling nanocomposite tectons},
  author={Zhang, Jianyuan and Santos, Peter J and Gabrys, Paul A and Lee, Sangho and Liu, Caroline and Macfarlane, Robert J},
  journal={Journal of the American Chemical Society},
  volume={138},
  number={50},
  pages={16228--16231},
  year={2016},
  publisher={ACS Publications}
}


@Article{Dreyfus2010,
  author        = {Dreyfus, Rémi and Leunissen, Mirjam E. and Sha, Roujie and Tkachenko, Alexei and Seeman, Nadrian C. and Pine, David J. and Chaikin, Paul M.},
  title         = {Aggregation-disaggregation transition of {DNA}-coated colloids: Experiments and theory},
  journal       = {Phys. Rev. E},
  year          = {2010},
  volume        = {81},
  number        = {4},
  pages         = {041404},
  month         = apr,
  publisher     = {American Physical Society},
  refid         = {10.1103/PhysRevE.81.041404},
}



@Article{Michele2013,
  author        = {Di Michele, Lorenzo and Eiser, Erika},
  title         = {Developments in understanding and controlling self assembly of {DNA}-functionalized colloids},
  journal       = {Phys. Chem. Chem. Phys.},
  year          = {2013},
  volume        = {15},
  number        = {9},
  pages         = {3115--3129},
  issn          = {1463-9076},
  abstract      = {In this article we review the latest achievements in understanding and controlling {DNA}-mediated interactions between colloidal particles. We report the results of experiments, theoretical studies and computer simulations designed to investigate interactions and aggregation/melting behaviour of {DNA}-functionalized colloids. The unprecedented insight into the physical effects influencing the interactions and their relation with the tunable parameters of the grafted {DNA} has resulted in innovative {DNA} coatings, which are expected to solve the decennial issues encountered in the self assembly of {DNA}-coated colloids.},
  publisher     = {The Royal Society of Chemistry},
}


@article{lowensohn2019linker,
  title={Linker-mediated phase behavior of DNA-coated colloids},
  author={Lowensohn, Janna and Oyarz{\'u}n, Bernardo and Paliza, Guillermo Narv{\'a}ez and Mognetti, Bortolo M and Rogers, W Benjamin},
  journal={Physical Review X},
  volume={9},
  number={4},
  pages={041054},
  year={2019},
  publisher={APS}
}

@Article{Harbage2016,
  author        = {Harbage, David and Kondev, Jané},
  title         = {Exact Length Distribution of Filamentous Structures Assembled from a Finite Pool of Subunits},
  journal       = {J. Phys. Chem. B},
  year          = {2016},
  volume        = {120},
  number        = {26},
  pages         = {6225--6230},
  month         = jul,
  issn          = {1520-6106},
  comment       = {doi: 10.1021/acs.jpcb.6b02242},
  doi           = {10.1021/acs.jpcb.6b02242},
  publisher     = {American Chemical Society},
}



@Article{Lenz2017,
  author        = {Lenz, Martin and Witten, Thomas A.},
  title         = {Geometrical frustration yields fibre formation in self-assembly},
  journal       = {Nature Physics},
  year          = {2017},
  volume        = {13},
  number        = {11},
  pages         = {1100--1104},
  month         = nov,
  issn          = {1745-2481},
  abstract      = {Deformable polygons are shown to form fibres when the energies associated with attraction and deformation are comparable. The fibres constitute a kinetically trapped metastable state, reminiscent of irreversible protein assembly in living systems.},
  refid         = {Lenz2017},
}



@Article{Sharma2014,
  author        = {Sharma, Prerna and Ward, Andrew and Gibaud, T. and Hagan, Michael F. and Dogic, Zvonimir},
  title         = {Hierarchical organization of chiral rafts in colloidal membranes},
  journal       = {Nature},
  year          = {2014},
  volume        = {513},
  number        = {7516},
  pages         = {77--80},
  month         = sep,
  issn          = {1476-4687},
  abstract      = {Inclusions dissolved in a colloidal membrane assemble into highly uniform finite-sized liquid droplets or rafts consisting of thousands of molecules.},
  refid         = {Sharma2014},
}



@Article{Miller2019,
  author        = {Miller, Joia M. and Joshi, Chaitanya and Sharma, Prerna and Baskaran, Arvind and Baskaran, Aparna and Grason, Gregory M. and Hagan, Michael F. and Dogic, Zvonimir},
  title         = {Conformational switching of chiral colloidal rafts regulates raft-raft attractions and repulsions},
  journal       = {Proc Natl Acad Sci USA},
  year          = {2019},
  volume        = {116},
  number        = {32},
  pages         = {15792},
  month         = aug,
  abstract      = {We describe hierarchical assemblages of colloidal rods that mimic some of the complexity and reconfigurability of biological structures. We show that chiral rod-like inclusions dissolved in an achiral colloidal membrane assemble into rafts, which are adaptable finite-sized liquid droplets that exhibit 2 distinct chiral states of opposite handedness. Interconverting between these 2 states switches the membrane-mediated raft interactions between long-ranged repulsions and attractions. Rafts with switchable interactions assemble into analogs of electrostatic complexation observed in charged particulate matter. Our results demonstrate a robust pathway for self-assembly of reconfigurable colloidal superstructures that does not depend on tuning the shape and interactions of the elemental units, but rather on the complexity of the emergent membrane-mediated interactions.Membrane-mediated particle interactions depend both on the properties of the particles themselves and the membrane environment in which they are suspended. Experiments have shown that chiral rod-like inclusions dissolved in a colloidal membrane of opposite handedness assemble into colloidal rafts, which are finite-sized reconfigurable droplets consisting of a large but precisely defined number of rods. We systematically tune the chirality of the background membrane and find that, in the achiral limit, colloidal rafts acquire complex structural properties and interactions. In particular, rafts can switch between 2 chiral states of opposite handedness, which alters the nature of the membrane-mediated raft-raft interactions. Rafts with the same chirality have long-ranged repulsions, while those with opposite chirality acquire attractions with a well-defined minimum. Both attractive and repulsive interactions are qualitatively explained by a continuum model that accounts for the coupling between the membrane thickness and the local tilt of the constituent rods. These switchable interactions enable assembly of colloidal rafts into intricate higher-order architectures, including stable tetrameric clusters and “ionic crystallites” of counter-twisting domains organized on a binary square lattice. Furthermore, the properties of individual rafts, such as their sizes, are controlled by their complexation with other rafts. The emergence of these complex behaviors can be rationalized purely in terms of generic couplings between compositional and orientational order of fluids of rod-like elements. Thus, the uncovered principles might have relevance for conventional lipid bilayers, in which the assembly of higher-order structures is also mediated by complex membrane-mediated interactions.},
}



@Article{Meng2014,
  author        = {Meng, Guangnan and Paulose, Jayson and Nelson, David R. and Manoharan, Vinothan N.},
  title         = {Elastic Instability of a Crystal Growing on a Curved Surface},
  journal       = {Science},
  year          = {2014},
  volume        = {343},
  number        = {6171},
  pages         = {634},
  month         = feb,
  abstract      = {When a material with a different set of lattice parameters is grown on the surface of a crystal of a second material, the stresses at the interface can affect the growing crystal. Meng et al. (p. 634) studied the growth of colloidal crystals on top of a curved water droplet. Owing to the elastic stress caused by the bending of the crystal, strong distortions occurred in the growing crystal, but, nonetheless, large single-crystalline domains with no topological defects were formed.Although the effects of kinetics on crystal growth are well understood, the role of substrate curvature is not yet established. We studied rigid, two-dimensional colloidal crystals growing on spherical droplets to understand how the elastic stress induced by Gaussian curvature affects the growth pathway. In contrast to crystals grown on flat surfaces or compliant crystals on droplets, these crystals formed branched, ribbon-like domains with large voids and no topological defects. We show that this morphology minimizes the curvature-induced elastic energy. Our results illustrate the effects of curvature on the ubiquitous process of crystallization, with practical implications for nanoscale disorder-order transitions on curved manifolds, including the assembly of viral capsids, phase separation on vesicles, and crystallization of tetrahedra in three dimensions.},
}

@Article{Crocker1996Colloid,
  author   = {John C. Crocker and David G. Grier},
  title    = {Methods of Digital Video Microscopy for Colloidal Studies},
  journal  = {Journal of Colloid and Interface Science},
  year     = {1996},
  volume   = {179},
  number   = {1},
  pages    = {298 - 310},
  issn     = {0021-9797},
  abstract = {We describe a set of image processing algorithms for extracting quantitative data from digitized video microscope images of colloidal suspensions. In a typical application, these direct imaging techniques can locate submicrometer spheres to within 10 nm in the focal plane and 150 nm in depth. Combining information from a sequence of video images into single-particle trajectories makes possible measurements of quantities of fundamental and practical interest such as diffusion coefficients and pair-wise interaction potentials. The measurements we describe in detail combine the outstanding resolution of digital imaging with video-synchronized optical trapping to obtain highly accurate and reproducible results very rapidly.},
  doi      = {https://doi.org/10.1006/jcis.1996.0217},
  keywords = {colloid, image processing, video microscopy, optical tweezers, dynamics, diffusion coefficient, interaction potential},
}

@article{ohnesorge1994density,
  title={Density functional theory of crystal-fluid interfaces and surface melting},
  author={Ohnesorge, R and L{\"o}wen, H and Wagner, H},
  journal={Physical review E},
  volume={50},
  number={6},
  pages={4801},
  year={1994},
  publisher={APS}
}

@book{phillips2012physical,
  title={Physical biology of the cell},
  author={Phillips, Rob and Kondev, Jane and Theriot, Julie and Garcia, Hernan},
  year={2012},
  publisher={Garland Science}
}

@Article{Sear2014CrystEngCom,
author ="Sear, Richard P.",
title  ="Quantitative studies of crystal nucleation at constant supersaturation: experimental data and models",
journal  ="CrystEngComm",
year  ="2014",
volume  ="16",
issue  ="29",
pages  ="6506-6522",
publisher  ="The Royal Society of Chemistry",
doi  ="10.1039/C4CE00344F",
}



@article{Mirkin2013Nature,
author = {Zhang, Chuan and Macfarlane, Robert and Young, Kaylie and Choi, Chung Hang and Hao, Liangliang and Auyeung, Evelyn and Liu, Guoliang and Zhou, Xiaozhu and Mirkin, Chad},
year = {2013},
month = {05},
pages = {},
title = {A general approach to {DNA}-programmable atom equivalents},
volume = {12},
journal = {Nature Materials},
doi = {10.1038/nmat3647}
}

@Article{Schultz1996Nature,
  author   = {Alivisatos, A. Paul and Johnsson, Kai P. and Peng, Xiaogang and Wilson, Troy E. and Loweth, Colin J. and Bruchez, Marcel P. and Schultz, Peter G.},
  title    = {Organization of 'nanocrystal molecules' using {DNA}},
  journal  = {Nature},
  year     = {1996},
  volume   = {382},
  number   = {6592},
  pages    = {609--611},
  month    = aug,
  issn     = {1476-4687},
  abstract = {PATTERNING matter on the nanometre scale is an important objective of current materials chemistry and physics. It is driven by both the need to further miniaturize electronic components and the fact that at the nanometre scale, materials properties are strongly size-dependent and thus can be tuned sensitively1. In nanoscale crystals, quantum size effects and the large number of surface atoms influence the, chemical, electronic, magnetic and optical behaviour2--4. 'Top-down' (for example, lithographic) methods for nanoscale manipulation reach only to the upper end of the nanometre regime5; but whereas 'bottom-up' wet chemical techniques allow for the preparation of mono-disperse, defect-free crystallites just 1-10 nm in size6-10, ways to control the structure of nanocrystal assemblies are scarce. Here we describe a strategy for the synthesis of'nanocrystal molecules', in which discrete numbers of gold nanocrystals are organized into spatially defined structures based on Watson-Crick base-pairing interactions. We attach single-stranded {DNA} oligonucleotides of defined length and sequence to individual nanocrystals, and these assemble into dimers and trimers on addition of a complementary single-stranded {DNA} template. We anticipate that this approach should allow the construction of more complex two-and three-dimensional assemblies.},
  groups   = {Intro},
  refid    = {Alivisatos1996},
}

@Article{Crocker2011SoftMatter,
  author    = {Scarlett, Raynaldo T. and Ung, Marie T. and Crocker, John C. and Sinno, Talid},
  title     = {A mechanistic view of binary colloidal superlattice formation using {DNA}-directed interactions},
  journal   = {Soft Matter},
  year      = {2011},
  volume    = {7},
  pages     = {1912-1925},
  abstract  = {The use of grafted{,} single-stranded {DNA} oligomer brushes with engineered sequences to effect tunable interactions between colloidal particles has now been demonstrated experimentally in both nano- and microscale systems. The versatility of this technology is highly appealing for realizing self-assembly of complex structures. However{,} ambiguities remain regarding how operating conditions{,} such as the rate at which the system temperature is reduced{,} interact with the other system parameters to produce crystalline assemblies with particular structures and defect densities. In this paper{,} a computational analysis is presented for the crystallization of binary superlattice crystals comprised of sub-micron colloidal spheres using a realistic model for the {DNA}-mediated interactions. The binary system consists of two populations of identical spheres that differ only in the sequence of the {DNA} oligomers grafted onto their surfaces. Metropolis Monte Carlo simulations and perturbation theory for free energy estimation are used to construct a detailed mechanistic picture for binary superlattice formation. The analysis reveals several interesting features of this system{,} particularly the role of kinetics in dictating not only the quality of the superlattice crystals{,} but also their crystalline structure. Using the results presented here{,} we make connections to recent experimental findings in similar binary crystallization systems.},
  doi       = {10.1039/C0SM00370K},
  groups    = {Intro},
  issue     = {5},
  publisher = {The Royal Society of Chemistry},
}

@Article{Crocker2005PhysRevLet,
  author    = {Biancaniello, Paul L. and Kim, Anthony J. and Crocker, John C.},
  title     = {Colloidal Interactions and Self-Assembly Using {DNA} Hybridization},
  journal   = {Phys. Rev. Lett.},
  year      = {2005},
  volume    = {94},
  pages     = {058302},
  month     = {Feb},
  doi       = {10.1103/PhysRevLett.94.058302},
  groups    = {Intro},
  issue     = {5},
  numpages  = {4},
  publisher = {American Physical Society},
}

@Article{Frenkel2001Nature,
  author   = {Auer, Stefan and Frenkel, Daan},
  title    = {Prediction of absolute crystal-nucleation rate in hard-sphere colloids},
  journal  = {Nature},
  year     = {2001},
  volume   = {409},
  number   = {6823},
  pages    = {1020--1023},
  month    = feb,
  issn     = {1476-4687},
  abstract = {Crystal nucleation is a much-studied phenomenon, yet the rate at which it occurs remains difficult to predict. Small crystal nuclei form spontaneously in supersaturated solutions, but unless their size exceeds a critical value--the so-called critical nucleus--they will re-dissolve rather than grow. It is this rate-limiting step that has proved difficult to probe experimentally. The crystal nucleation rate depends on Pcrit, the (very small) probability that a critical nucleus forms spontaneously, and on a kinetic factor (κ) that measures the rate at which critical nuclei subsequently grow. Given the absence of a priori knowledge of either quantity, classical nucleation theory1 is commonly used to analyse crystal nucleation experiments, with the unconstrained parameters adjusted to fit the observations. This approach yields no ‘first principles’ prediction of absolute nucleation rates. Here we approach the problem from a different angle, simulating the nucleation process in a suspension of hard colloidal spheres, to obtain quantitative numerical predictions of the crystal nucleation rate. We find large discrepancies between the computed nucleation rates and those deduced from experiments2,3,4: the best experimental estimates of Pcrit seem to be too large by several orders of magnitude.},
  groups   = {Intro},
  refid    = {Auer2001},
}

@Article{Crocker2017PhysRevLett,
  author    = {Jenkins, Ian C. and Crocker, John C. and Sinno, Talid},
  title     = {Interaction Heterogeneity can Favorably Impact Colloidal Crystal Nucleation},
  journal   = {Phys. Rev. Lett.},
  year      = {2017},
  volume    = {119},
  pages     = {178002},
  month     = {Oct},
  doi       = {10.1103/PhysRevLett.119.178002},
  groups    = {Intro},
  issue     = {17},
  numpages  = {6},
  publisher = {American Physical Society},
}

@Article{Buzzaccaro2007PhysRevLett,
  author    = {Buzzaccaro, Stefano and Rusconi, Roberto and Piazza, Roberto},
  title     = {``Sticky'' Hard Spheres: Equation of State, Phase Diagram, and Metastable Gels},
  journal   = {Phys. Rev. Lett.},
  year      = {2007},
  volume    = {99},
  pages     = {098301},
  month     = {Aug},
  doi       = {10.1103/PhysRevLett.99.098301},
  groups    = {Intro},
  issue     = {9},
  numpages  = {4},
  publisher = {American Physical Society},
}

@Article{Taborek1985PhysRevB,
  author    = {Taborek, P.},
  title     = {Nucleation in emulsified supercooled water},
  journal   = {Phys. Rev. B},
  year      = {1985},
  volume    = {32},
  pages     = {5902--5906},
  month     = {Nov},
  doi       = {10.1103/PhysRevB.32.5902},
  groups    = {Intro},
  issue     = {9},
  numpages  = {0},
  publisher = {American Physical Society},
}

@Article{SantaLucia2004RevOfBioPhys,
  author   = {SantaLucia, John and Hicks, Donald},
  title    = {The Thermodynamics of {DNA} Structural Motifs},
  journal  = {Annual Review of Biophysics and Biomolecular Structure},
  year     = {2004},
  volume   = {33},
  number   = {1},
  pages    = {415-440},
  abstract = { ▪ Abstract {DNA} secondary structure plays an important role in biology, genotyping diagnostics, a variety of molecular biology techniques, in vitro–selected {DNA} catalysts, nanotechnology, and {DNA}-based computing. Accurate prediction of {DNA} secondary structure and hybridization using dynamic programming algorithms requires a database of thermodynamic parameters for several motifs including Watson-Crick base pairs, internal mismatches, terminal mismatches, terminal dangling ends, hairpins, bulges, internal loops, and multibranched loops. To make the database useful for predictions under a variety of salt conditions, empirical equations for monovalent and magnesium dependence of thermodynamics have been developed. Bimolecular hybridization is often inhibited by competing unimolecular folding of a target or probe {DNA}. Powerful numerical methods have been developed to solve multistate-coupled equilibria in bimolecular and higher-order complexes. This review presents the current parameter set available for making accurate {DNA} structure predictions and also points to future directions for improvement. },
  groups   = {Intro},
}


@article{Frenkel2007JournalChemPhys,
author = {Charbonneau,P.  and Frenkel,D. },
title = {Gas-solid coexistence of adhesive spheres},
journal = {The Journal of Chemical Physics},
volume = {126},
number = {19},
pages = {196101},
year = {2007},
doi = {10.1063/1.2737051},

}


@Article{Megen1997PhysRevE,
  author    = {Harland, J. L. and van Megen, W.},
  title     = {Crystallization kinetics of suspensions of hard colloidal spheres},
  journal   = {Phys. Rev. E},
  year      = {1997},
  volume    = {55},
  pages     = {3054--3067},
  month     = {Mar},
  doi       = {10.1103/PhysRevE.55.3054},
  groups    = {Intro},
  issue     = {3},
  numpages  = {0},
  publisher = {American Physical Society},
}

@Article{Palberg1999CondensedMatter,
  author    = {Thomas Palberg},
  title     = {Crystallization kinetics of repulsive colloidal spheres},
  journal   = {Journal of Physics: Condensed Matter},
  year      = {1999},
  volume    = {11},
  number    = {28},
  pages     = {R323--R360},
  month     = {jan},
  abstract  = {Colloidal spheres interacting via a purely repulsive potential provide an excellent model system to study the kinetics of solidification from the melt. Such systems are readily accessible by comparably simple yet powerful optical methods like time resolved static light scattering and microscopy, reviewed in the first part of this paper. We then present results from our own recent studies within a framework of data available from literature. In particular we investigated nucleation and growth of hard sphere crystals using combined Bragg and small angle light scattering and of charged sphere crystals using Bragg microscopy. Special attention is given to the range of validity of classical nucleation theory and of Wilson Frenkel growth and a discussion of kinetic prefactors for both processes.},
  doi       = {10.1088/0953-8984/11/28/201},
  groups    = {Intro},
  publisher = {{IOP} Publishing},
}

@Article{Ackerson1993PhysRevE,
  author    = {Sch\"atzel, Klaus and Ackerson, Bruce J.},
  title     = {Density fluctuations during crystallization of colloids},
  journal   = {Phys. Rev. E},
  year      = {1993},
  volume    = {48},
  pages     = {3766--3777},
  month     = {Nov},
  doi       = {10.1103/PhysRevE.48.3766},
  groups    = {Intro},
  issue     = {5},
  numpages  = {0},
  publisher = {American Physical Society},
}

@Article{KunTa2013PhysRevE,
  author    = {Wu, Kun-Ta and Feng, Lang and Sha, Ruojie and Dreyfus, R\'emi and Grosberg, Alexander Y. and Seeman, Nadrian C. and Chaikin, Paul M.},
  title     = {Kinetics of {DNA}-coated sticky particles},
  journal   = {Phys. Rev. E},
  year      = {2013},
  volume    = {88},
  pages     = {022304},
  month     = {Aug},
  doi       = {10.1103/PhysRevE.88.022304},
  issue     = {2},
  numpages  = {8},
  publisher = {American Physical Society},
}

@PhdThesis{Duij1994Utrecth,
  author = {Jeroen van Duijneveldt},
  title  = {Phase Transitions In Colloidal Suspensions},
  school = {Universiteit Utrecth},
  year   = {1994},
}

@Article{Frenkel2004Nature,
  author   = {Cacciuto, A. and Auer, S. and Frenkel, D.},
  title    = {Onset of heterogeneous crystal nucleation in colloidal suspensions},
  journal  = {Nature},
  year     = {2004},
  volume   = {428},
  number   = {6981},
  pages    = {404--406},
  month    = mar,
  issn     = {1476-4687},
  abstract = {The addition of small ‘seed’ particles to a supersaturated solution can greatly increase the rate at which crystals nucleate. This process is understood, at least qualitatively, when the seed has the same structure as the crystal that it spawns1,2. However, the microscopic mechanism of seeding by a ‘foreign’ substance is not well understood. Here we report numerical simulations of colloidal crystallization seeded by foreign objects. We perform Monte Carlo simulations to study how smooth spherical seeds of various sizes affect crystallization in a suspension of hard colloidal particles. We compute the free-energy barrier associated with crystal nucleation3,4. A low barrier implies that nucleation is easy. We find that to be effective crystallization promoters, the seed particles need to exceed a well-defined minimum size. Just above this size, seed particles act as crystallization ‘catalysts’ as newly formed crystallites detach from the seed. In contrast, larger seed particles remain covered by the crystallites that they spawn. This phenomenon should be experimentally observable and can have important consequences for the control of the resulting crystal size distribution.},
  refid    = {Cacciuto2004},
}

@article{Anna2003FormationOD,
author = {Anna,Shelley L.  and Bontoux,Nathalie  and Stone,Howard A. },
title = {Formation of dispersions using flow focusing in microchannels},
journal = {Applied Physics Letters},
volume = {82},
number = {3},
pages = {364-366},
year = {2003},
doi = {10.1063/1.1537519},

}

@Article{Rogers2011PNAS,
  author    = {Rogers, W. Benjamin and Crocker, John C.},
  title     = {Direct measurements of {DNA}-mediated colloidal interactions and their quantitative modeling},
  journal   = {Proceedings of the National Academy of Sciences of the United States of America},
  year      = {2011},
  volume    = {108},
  number    = {38},
  pages     = {15687--15692},
  issn      = {00278424},
  abstract  = {{DNA} bridging can be used to induce specific attractions between small particles, providing a highly versatile approach to creating unique particle-based materials having a variety of periodic structures. Surprisingly, given the fact that the thermodynamics of {DNA} strands in solution are completely understood, existing models for {DNA}-induced particle interactions are typically in error by more than an order of magnitude in strength and a factor of two in their temperature dependence. This discrepancy has stymied efforts to design the complex temperature, sequence and time-dependent interactions needed for the most interesting applications, such as materials having highly complex or multicomponent microstructures or the ability to reconfigure or self-replicate. Here we report high-spatial resolution measurements of {DNA}-induced interactions between pairs of polystyrene microspheres at binding strengths comparable to those used in self-assembly experiments, up to 6 kBT. We also describe a conceptually straightforward and numerically tractable model that quantitatively captures the separation dependence and temperature-dependent strength of these {DNA}-induced interactions, without empirical corrections. This model was equally successful when describing the more complex and practically relevant case of grafted {DNA} brushes with self-interactions that compete with interparticle bridge formation. Together, our findings motivate a nanomaterial design approach where unique functional structures can be found computationally and then reliably realized in experiment.},
  database  = {JSTOR},
  publisher = {National Academy of Sciences},
}


@Article{Weitz2001Science,
  author   = {Gasser, U. and Weeks, Eric R. and Schofield, Andrew and Pusey, P. N. and Weitz, D. A.},
  title    = {Real-Space Imaging of Nucleation and Growth in Colloidal Crystallization},
  journal  = {Science},
  year     = {2001},
  volume   = {292},
  number   = {5515},
  pages    = {258},
  month    = apr,
  abstract = {Crystallization of concentrated colloidal suspensions was studied in real space with laser scanning confocal microscopy. Direct imaging in three dimensions allowed identification and observation of both nucleation and growth of crystalline regions, providing an experimental measure of properties of the nucleating crystallites. By following their evolution, we identified critical nuclei, determined nucleation rates, and measured the average surface tension of the crystal-liquid interface. The structure of the nuclei was the same as the bulk solid phase, random hexagonal close-packed, and their average shape was rather nonspherical, with rough rather than faceted surfaces.},
}

@Article{Fan2011NanoLetters,
  author    = {Jonathan A. Fan and Yu He and Kui Bao and Chihhui Wu and Jiming Bao and Nicholas B. Schade and Vinothan N. Manoharan and Gennady Shvets and Peter Nordlander and David R. Liu and Federico Capasso},
  title     = {{DNA}-Enabled Self-Assembly of Plasmonic Nanoclusters},
  journal   = {Nano Letters},
  year      = {2011},
  volume    = {11},
  number    = {11},
  pages     = {4859--4864},
  month     = {nov},
  doi       = {10.1021/nl203194m},
  file      = {:nl203194m.pdf:PDF},
  publisher = {American Chemical Society ({ACS})},
}

@Article{Cong2013CSR,
  author    = {Cong, Hailin and Yu, Bing and Tang, Jianguo and Li, Zejing and Liu, Xuesong},
  title     = {Current status and future developments in preparation and application of colloidal crystals},
  journal   = {Chem. Soc. Rev.},
  year      = {2013},
  volume    = {42},
  pages     = {7774-7800},
  abstract  = {Colloidal crystals (CCs) are ordered arrays of monodisperse colloidal particles. Because of the presence of a periodic superlattice of colloids and voids{,} CCs bear many unique structures and fascinating properties which are distinctly different from those of standard crystals with atoms{,} ions or molecules as repeating subunits. The research on CCs has surprisingly blossomed during recent decades{,} and many practical materials based on CCs with potential applications in photonic devices{,} material science and biomedical engineering have been generated. In this review{,} we give a systematic{,} balanced and comprehensive summary of the main aspects of CCs related to their preparation and application{,} and propose perspectives for the future developments of CCs.},
  doi       = {10.1039/C3CS60078E},
  issue     = {19},
  publisher = {The Royal Society of Chemistry},
}

@Article{theBigMan1905,
  author  = {Einstein, A.},
  title   = {Über die von der molekularkinetischen Theorie der Wärme geforderte Bewegung von in ruhenden Flüssigkeiten suspendierten Teilchen},
  journal = {Annalen der Physik},
  year    = {1905},
  volume  = {322},
  number  = {8},
  pages   = {549-560},
  doi     = {10.1002/andp.19053220806},
}

@article{heymann2014room,
  title={Room-temperature serial crystallography using a kinetically optimized microfluidic device for protein crystallization and on-chip X-ray diffraction},
  author={Heymann, Michael and Opthalage, Achini and Wierman, Jennifer L and Akella, Sathish and Szebenyi, Doletha ME and Gruner, Sol M and Fraden, Seth},
  journal={IUCrJ},
  volume={1},
  number={5},
  pages={349--360},
  year={2014},
  publisher={International Union of Crystallography}
}

@article{galkin1999direct,
  title={Direct determination of the nucleation rates of protein crystals},
  author={Galkin, Oleg and Vekilov, Peter G},
  journal={The Journal of Physical Chemistry B},
  volume={103},
  number={49},
  pages={10965--10971},
  year={1999},
  publisher={ACS Publications}
}

@article{akella2014emulsion,
  title={Emulsion-based technique to measure protein crystal nucleation rates of lysozyme},
  author={Akella, Sathish V and Mowitz, Aaron and Heymann, Michael and Fraden, Seth},
  journal={Crystal Growth \& Design},
  volume={14},
  number={9},
  pages={4487--4509},
  year={2014},
  publisher={ACS Publications}
}

@article{dombrowski2010modeling,
  title={Modeling the crystallization of proteins and small organic molecules in nanoliter drops},
  author={Dombrowski, Richard D and Litster, James D and Wagner, Norman J and He, Yinghe},
  journal={AIChE journal},
  volume={56},
  number={1},
  pages={79--91},
  year={2010},
  publisher={Wiley Online Library}
}

@article{palberg1999crystallization,
  title={Crystallization kinetics of repulsive colloidal spheres},
  author={Palberg, Thomas},
  journal={Journal of Physics: Condensed Matter},
  volume={11},
  number={28},
  pages={R323},
  year={1999},
  publisher={IOP Publishing}
}

@article{charbonneau2007gas,
  title={Gas-solid coexistence of adhesive spheres},
  author={Charbonneau, Patrick and Frenkel, D},
  journal={The Journal of Chemical Physics},
  volume={126},
  number={19},
  pages={196101},
  year={2007},
  publisher={American Institute of Physics}
}

@article{libbrecht2003growth,
  title={Growth rates of the principal facets of ice between $-10^\circ${C} and $-40^\circ${C}},
  author={Libbrecht, Kenneth G},
  journal={Journal of Crystal Growth},
  volume={247},
  number={3-4},
  pages={530--540},
  year={2003},
  publisher={Elsevier}
}

@article{sear2007nucleation,
  title={Nucleation: {T}heory and applications to protein solutions and colloidal suspensions},
  author={Sear, Richard P},
  journal={Journal of Physics: Condensed Matter},
  volume={19},
  number={3},
  pages={033101},
  year={2007},
  publisher={IOP Publishing}
}

@article{jacobs2016self,
  title={Self-assembly of structures with addressable complexity},
  author={Jacobs, William M and Frenkel, Daan},
  journal={Journal of the American Chemical Society},
  volume={138},
  number={8},
  pages={2457--2467},
  year={2016},
  publisher={ACS Publications}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

@article{Fraden2009,
author = {Selimović, Šeila and Jia, Yanwei and Fraden, Seth},
title = {Measuring the Nucleation Rate of Lysozyme using Microfluidics},
journal = {Crystal Growth \& Design},
volume = {9},
number = {4},
pages = {1806-1810},
year = {2009},
doi = {10.1021/cg800990k},
}

@article{Pound1952JACS,
author = {Pound, Guy M. and Mer, Victor K. La},
title = {Kinetics of Crystalline Nucleus Formation in Supercooled Liquid Tin},
journal = {Journal of the American Chemical Society},
volume = {74},
number = {9},
pages = {2323-2332},
year = {1952},
doi = {10.1021/ja01129a044},

}
